Reply to 'Comments on Graphon Signal Processing' [arXiv:2310.14683]

This technical note addresses an issue [arXiv:2310.14683] with the proof (but not the statement) of [arXiv:2003.05030, Proposition 4]. The statement of the proposition is correct, but the proof as written in [arXiv:2003.05030] is not and due to a typo in the manuscript, a reference to the correct proof is effectively missing. In the sequel, we present [arXiv:2003.05030, Proposition 4] and its proof. The proof follows from results in [2] that we reproduce here for clarity of exposition. Since the statement of the proposition remains correct, no change in the results of [arXiv:2003.05030] are required. In particular, Lemma 3 and Lemma 4 showing spectral convergence of graphs to graphons, Theorem 1 showing convergence of the GFT to the WFT, and Theorems 3 and 4 showing convergence of graph to graphon filters, remain valid.

==> figures/figures/1030/10_filter_convergence.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex


\def \thisplotscale {1.0}
\def \unit {\thisplotscale cm}

\tikzstyle {block blue} = [ block, 
                            thin,
                            minimum width  = 2.8*\unit, 
                            minimum height = 1.3*\unit, 
                            anchor = west,
                            fill = blue!15]

\tikzstyle {block green} = [ block blue, 
                             fill = mygreen!25]

\tikzstyle {block gray} = [ block blue, 
                            fill = black!15]


\def \deltax      {+1.0}
\def \deltaother  {+0.7}

\def \graphfilter   {
                      % \only<2- | handout : 1> 
                       %   {\bie \bbH(\bbS_n) = \sum_{k=1}^{K} \red{h_k} \bbS_n^{k}  \eie}
                        \only<2- | handout : 1> 
                          {\bie \bby_n = \sum_{k=1}^{K} \red{h_k} \bbS_n^{k} \bbx_n \eie}
                    }

\def \graphonfilter {
                       %\only<2-7 | handout : 1> 
                        %  {\bie T_H = \sum_{k=1}^{K} \red{h_k} T_\bbW^{(k)}  \eie}
                        \only<3-  | handout : 1> 
                          {\bie \bby_n = \sum_{k=1}^{K} \red{h_k} T_\bbW^{(k)} X  \eie}
                    }

{\footnotesize

\begin{tikzpicture}[x = 1*\unit, y = 1*\unit]


   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % GFT chain
   
   % Begin by drawing an empty node for initializing the chain
   \node (T0) [] {};

   % Draw the chain of graph shifts. 
   \os{2-}{\path (T0.east) ++ (\deltax, 0) node (T1) [block green] {\graphfilter};}

   % End by drawing an empty node at the end of the chain
   \path (T1.east) ++ (\deltax, 0) node (T2) [] {};
   
   % Draw the arrows connecting the blocks
   \os{2-}{\path[-stealth, draw] (T0) -- (T1) node [near start, above] {$\bbx_n$};}	
   \os{2-}{\path[-stealth, draw] (T1) -- (T2) node [near end,   above] {$\bby_n$};}	   

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % WFT chain
   
   % Begin by drawing an empty node for initializing the chain
   \path (T2.east) ++ (\deltaother, 0) node (B0) [] {};

   % Draw the chain of graph shifts. 
   \os{3-}{\path (B0.east) ++ (\deltax, 0) node (B1) [block blue] {\graphonfilter};}

   % End by drawing an empty node at the end of the chain
   \path (B1.east) ++ (\deltax, 0) node (B2) [] {};
   
   % Draw the arrows connecting the blocks
   \os{3-}{\path[-stealth, draw] (B0) -- (B1) node [near start, above] {$X$};}	
   \os{3-}{\path[-stealth, draw] (B1) -- (B2) node [near end,   above] {$Y$};}	   


\end{tikzpicture}

}

        


==> figures/figures/1030/23_low_pass_lipschitz_filter.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}

\def \frequencyresponse 
     { 0.1*exp(-(1*(x-4.3))^2) 
       + 0.25*exp(-(2*(x-4.5))^2) 
       + 0.37*exp(-(1.3*(x-6.5))^2) 
       + 0.55}
       
\def \flatfrequencyresponse 
     { 0.}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 enlarge x limits = false,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=otimes*, 
          mark options={black}]
         {\frequencyresponse};
         
\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};

\end{axis}

\end{tikzpicture}

}



==> figures/figures/1030/26_low_pass_lipschitz_filter_high_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}

\def \frequencyresponse 
     { 0.1*exp(-(1*(x-4.3))^2) 
       + 0.25*exp(-(2*(x-4.5))^2) 
       + 0.37*exp(-(1.3*(x-6.5))^2) 
       + 0.55}
       
\def \flatfrequencyresponse 
     { 0.}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 enlarge x limits = false,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             enlarge x limits=false,             					
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57}, 
          color = blue!30, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!30}]
         {\frequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4}, 
          color = mygreen!30, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!30}]
         {\frequencyresponse};

         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=otimes*, 
          mark options={black}]
         {\frequencyresponse};
         
\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};

%   \addlegendentry{\scriptsize $\bbW$}
%   \addlegendentry{\scriptsize $\bbG_n$}

\end{axis}

\end{tikzpicture}

}



==> figures/figures/1030/43_constant_filter.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/43_high_pass_filter.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}
     
            
\def \flatfrequencyresponsezero 
     { 0.0}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponsezero};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black}]
         {\flatfrequencyresponsezero};

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/46_constant_filter_graphon_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57, 
              2.63, 3, 4.24, 5.51, 6.72, 7.6}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4, 2.5, 3.13, 4.13, 
              5.68, 6.87, 7.8}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};

%   \addlegendentry{\scriptsize $\bbW$}
%   \addlegendentry{\scriptsize $\bbG_n$}

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/49_constant_filter_zeroc_graphon_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}
     
\def \flatfrequencyresponsezero 
     { 0.0}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};
         
\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponsezero};
         
\addplot+[samples at = {2.1}, 
          mark=otimes*, 
          mark options={black}]
         {\flatfrequencyresponsezero};

%   \addlegendentry{\scriptsize $\bbW$}
%   \addlegendentry{\scriptsize $\bbG_n$}

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/49_high_pass_filter_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}
     
            
\def \flatfrequencyresponsezero 
     { 0.0}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]
             
\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\flatfrequencyresponse};
         
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black}]
         {\flatfrequencyresponsezero};

         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponsezero};
         

         


\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/49_high_pass_filter_eig__1_.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57, 
              2.63, 3, 4.24, 5.51, 6.72, 7.6}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4, 2.5, 3.13, 4.13, 
              5.68, 6.87, 7.8}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};

%   \addlegendentry{\scriptsize $\bbW$}
%   \addlegendentry{\scriptsize $\bbG_n$}

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/63_variable_band_filter.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}

\def \frequencyresponse 
     { 0.1*exp(-(1*(x-4.3))^2) 
       + 0.25*exp(-(2*(x-4.5))^2) 
       + 0.37*exp(-(1.3*(x-6.5))^2) 
       + 0.55}
       
\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 enlarge x limits = false,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,            					
             legend pos=north east,
             legend columns=3]
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};

\end{axis}

\end{tikzpicture}

}



==> figures/figures/1030/66_variable_band_filter_graphon_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}

\def \frequencyresponse 
     { 0.1*exp(-(1*(x-4.3))^2) 
       + 0.25*exp(-(2*(x-4.5))^2) 
       + 0.37*exp(-(1.3*(x-6.5))^2) 
       + 0.55}
       
\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 enlarge x limits = false,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,            					
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57, 
              2.63, 3, 4.24, 5.51, 6.72, 7.6}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\frequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4, 2.5, 3.13, 4.13, 
              5.68, 6.87, 7.8}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\frequencyresponse};
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};

\end{axis}

\end{tikzpicture}

}



==> figures/figures/macros/0_annotate_plot.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with coordinates given 
      
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

   % Annotate axis
   \node at (\xmax*\xfactor - \xmin*\xfactor, -\ydeltaskip*\yfactor) 
            [anchor = south west] 
            {$\lam_{\phantom{1}}$};

   \node at (\xmin*\xfactor, -0.14*\yfactor) 
            [anchor = south east] 
            {$\phantom{\lam_{\phantom{1}}}$};


   \node at (\xmin*\xfactor, \ymax*\yfactor) 
            [anchor = east] 
            {$\tdh(\lam)~$};

   \node at (\xmax*\xfactor - \xmin*\xfactor, \ymax*\yfactor) 
            [anchor = west] 
            {$\phantom{~{\tdh(\lam)}}$};


            
   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationthree};

   % Next three annotations. Associated with another signal
   \node at (\annotatedfour*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationfour};

   \node at (\annotatedfive*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationfive};

   \node at (\annotatedsix*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationsix};
   








==> figures/figures/macros/0_annotate_plot_no_axes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with coordinates given 
      
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

            
   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationthree};

   % Next three annotations. Associated with another signal
   \node at (\annotatedfour*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationfour};

   \node at (\annotatedfive*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationfive};

   \node at (\annotatedsix*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationsix};
   








==> figures/figures/macros/0_draw_filter.tex <==
% Plot filter with a black thick line  

\addplot[ domain     = \xmin:\xmax,
          samples    = 150, 
          color      = black!99,
          line width = 1.2]
          { \filter };



==> figures/figures/macros/0_draw_gaussian_macro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Code for drawing Gaussian filter
% 
\newcommand{\drawgaussian}[7]
{
   \def \filter { ( \height*exp(-(1/\width*(x-\center))^2) ) }
   \def \center {#1}
   \def \width  {#2}
   \def \height {#3}

   \def \xminhere   {#4}
   \def \xmaxhere   {#5}

   % Draw filter Three
   \addplot[ domain     = \center-3.0*\width:\center + 3.0*\width, 
             samples    = 80, 
             color      = #6,
             line width = #7]
           { \filter };

   \addplot[ domain     = \xminhere:\center-3.0*\width, 
             samples    = 2, 
             color      = #6,
             line width = #7]
           { 0 };
   
   \addplot[ domain     = \center+3.0*\width:\xmaxhere, 
             samples    = 2, 
             color      = #6,
             line width = #7]
           { 0 };
}


==> figures/figures/macros/0_draw_gft_blue.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plot GFT input and GFT ouptut at given spikes

   % Plot input spikes. Make them all of height 1
   \addplot+[ samples at   = \spikes, 
              ycomb, 
              mark         = otimes*, 
              color        =  blue!20, 
              mark options = {blue!20}
            ]
            { \ymax };

   %Plot frequency response spikes
   \addplot+[ samples at   = \spikes, 
              solid, 
              ycomb, 
              mark         = otimes*, 
              line width   = 1.2,              
              color        =  blue!60, 
              mark options = {blue!60}
            ]
            { \GFT*\filter};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with three coordinates given 
   
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationthree};








==> figures/figures/macros/0_draw_gft_mygreen.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plot GFT input and GFT ouptut at given spikes

   % Plot input spikes. Make them all of height 1
   \addplot+[ samples at   = \spikes, 
              ycomb, 
              mark         = otimes*, 
              color        =  mygreen!20, 
              mark options = {mygreen!20}
            ]
            { \ymax };

   %Plot frequency response spikes
   \addplot+[ samples at   = \spikes, 
              solid, 
              ycomb, 
              mark         = otimes*, 
              line width   = 1.2,              
              color        =  mygreen!60, 
              mark options = {mygreen!60}
            ]
            { \GFT*\filter};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with three coordinates given 
   
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationthree};








==> figures/figures/macros/0_draw_gft_red.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plot GFT input and GFT ouptut at given spikes

   % Plot input spikes. Make them all of height 1
   \addplot+[ samples at   = \spikes, 
              ycomb, 
              mark         = otimes*, 
              color        =  red!20, 
              mark options = {red!20}
            ]
            { \ymax };

   %Plot frequency response spikes
   \addplot+[ samples at   = \spikes, 
              solid, 
              ycomb, 
              mark         = otimes*, 
              line width   = 1.2,              
              color        =  red!60, 
              mark options = {red!60}
            ]
            { \GFT*\filter};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with three coordinates given 
   
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationthree};








==> figures/figures/macros/0_draw_shade.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro to draw shadings in the background to highlight 
% eigenvalues that are moving 
 
   \newcommand{\drawshade}[3]
   {
      \path [fill = #3] 
            ( #1*\xfactor - \xmin*\xfactor - 5.0, 0.0*\yfactor) rectangle 
            ( #2*\xfactor - \xmin*\xfactor + 5.0, 1.0*\yfactor);
   }


